Learning Shared Representations in Multi-task Reinforcement Learning

We investigate a paradigm in multi-task reinforcement learning (MT-RL) in which an agent is placed in an environment and needs to learn to perform a series of tasks, within this space. Since the environment does not change, there is potentially a lot of common ground amongst tasks and learning to solve them individually seems extremely wasteful. In this paper, we explicitly model and learn this shared structure as it arises in the state-action value space. We will show how one can jointly learn optimal value-functions by modifying the popular Value-Iteration and Policy-Iteration procedures to accommodate this shared representation assumption and leverage the power of multi-task supervised learning. Finally, we demonstrate that the proposed model and training procedures, are able to infer good value functions, even under low samples regimes. In addition to data efficiency, we will show in our analysis, that learning abstractions of the state space jointly across tasks leads to more robust, transferable representations with the potential for better generalization. this shared representation assumption and leverage the power of multi-task supervised learning. Finally, we demonstrate that the proposed model and training procedures, are able to infer good value functions, even under low samples regimes. In addition to data efficiency, we will show in our analysis, that learning abstractions of the state space jointly across tasks leads to more robust, transferable representations with the potential for better generalization.

==> MTPI.tex <==
\section{Multi-task Policy Iteration}
In this section, we will make a similar argument as the one presented in the last section for MT-FQI, to extend the framework of \textit{general policy iteration} to the MT-RL scenario. As outlined previously, policy iteration algorithms rely on an alternating procedure between a policy evaluation step and a policy improvement step. We can extend this framework to the multi-task case, by defining a (current) set of policies $\Pi = \{\pi_t\}_{t=1}^T$, one for each task, and then we evolve this set of policies jointly at each iteration, $k$. Please find a detailed outline of the proposed procedure in Algorithm \ref{alg:MT-PI}. For now, we implement the policy improvement step by acting greedily with respect to our current estimates of the value function. This step is done individually for each task. 

% ===========================================================================================
\begin{algorithm}                      % enter the algorithm environment
\caption{Joint Multi-Task Policy Iteration (MT-PI)}          % give the algorithm a caption
\label{alg:MT-PI}                           % and a label for \ref{} commands later in the document
\begin{algorithmic}                    % enter the algorithmic environment
% ===========================================================================================
\REQUIRE $\mathcal{D} = \cup_{t=1}^T \mathcal{D}_t$, set of experiences for each task $t$
\vspace{1em}
 
\STATE \textbf{Initialize} $\Theta = \Theta_0, k = 0$
\vspace{1em}

\WHILE{convergence not reached $(d\Theta< \epsilon || k < \text{MaxIter})$}
\STATE \textbf{Policy Evaluation}:
 \\ Compute $\Theta^{(k)} =$ MT-PE($ \mathcal{D}, \Pi^{(k)}$) implemented in Algorithm \ref{alg:MT-PE} \\ where  $\Pi^{(k)} = \left[ {\pi_1}, \cdots,{\pi_t}, \cdots, {\pi_T} \right]$ and $\Theta^{(k)} = \left[ \theta^{\pi_1}_1, \cdots, \theta^{\pi_t}_t, \cdots, \theta^{\pi_T}_T \right]$

\STATE \textbf{Policy Improvement} 
 \\ $\pi_j^{(k+1)}(a|s) = \arg \max_a{Q^{\pi^{(k)}_t}_{t}(s,a)} = \arg \max_a{f_{\theta^{\pi_t}_t}(s,a)}$

\ENDWHILE

\vspace{1em}
\STATE \textbf{Return:} $\Theta = \{\theta_t\}_{t=1}^T$ and learnt policies $\Pi = \{\pi_t\}_{t=1}^T \approx \Pi^*$
\end{algorithmic}
\end{algorithm}
% ===========================================================================================
On the other hand, we allow joint learning and sharing of knowledge in the policy evaluation step. This gives rise to a general procedure we will call Multi-task Policy Evaluation (MT-PE)- see Algorithm \ref{alg:MT-PE}.  In MT-PE, we are given a set of policies $\Pi = \{\pi_t\}_{t=1}^T$, one for each task, and a collection of experiences $\mathcal{D}= \cup_{t=1}^T \mathcal{D}_t$. Then the aim of the algorithm is to approximate the corresponding value functions $Q^{\pi_t}_t$ associated with acting out policy $\pi_t$ for task $t$. Note that in general, this step (policy evaluation) will require on-policy data, for each policy $\pi_t$ and for each task $t$. This could be quite demanding and inefficient data-wise, as the numbers of tasks grow, not to mention this is just the inner loop of another iterative algorithm (MT-PI). In this work, we present an implementation of policy evaluation that circumvents this problem. 

Making use of the Bellman Expectation Equation and following the same arguments as for FQI, we can now compute regression targets for approximating $\{Q^{\pi_t}_t\}$. Therefore, we have now reduced the original problem to a set of regression problems that can be solved jointly, under a shared input space representation. This is very similar to the multi-task learning step employed in MT-FQI, but now the shared structure is learnt to model the input set of policies $\Pi = \{\pi_t\}_{t=1}^T$, rather than the optimal ones. Nevertheless, by constantly improving the set of policies that are presented to the MT-PE step, we should eventually be able to convergence to the optimal policies and thus at this point, the policy evaluation step should be able to recover the shared structure amongst optimal value functions.

% ===========================================================================================
\begin{algorithm}                      % enter the algorithm environment
\caption{Multi-Task Policy Evaluation (MT-PE)}          % give the algorithm a caption
\label{alg:MT-PE}                           % and a label for \ref{} commands later in the document
% ===========================================================================
\begin{algorithmic}                    % enter the algorithmic environment
\REQUIRE $\mathcal{D} = \cup_{t=1}^T \mathcal{D}_t$, set of experiences for each task $t$ 
\\ A set of policies $\Pi =  \{\pi_t\}_{t=1}^T$, for each task $t$ that need to be evaluated
\vspace{1em}

\STATE \textbf{Initialize} $\Theta = \Theta_0, i = 0$
\vspace{1em}

\WHILE{convergence not reached $(d\Theta< \epsilon || k< \text{MaxIter})$}
\STATE \textbf{Compute Targets}:
 \\ $ \mathcal{Y}_t^{(i+1)} = \{ y_t^{(i+1)}(s,a) = R_t(s,a) + \gamma Q^{(i)}_t(s',\pi_t(s'))|(s,a,s') \in \mathcal{D}_t \}, \forall t = 1,T$ \\

\STATE \textbf{Multi-task Learning:}  
 \\ $\Theta^{(i+1)} = \text{MTL}(\mathcal{D} = \cup_{t=1}^T \mathcal{D}_t, \mathcal{Y}^{(i)} = \cup_{t=1}^T \mathcal{Y}_t^{(i)})$ %via Eq. \ref{eq: MTL1}
 \\
 
 \STATE  $d\Theta = \Vert \Theta^{(i+1)} - \Theta^{(i)} \Vert, i=i+1$ 
\ENDWHILE

\vspace{1em}
\STATE \textbf{Return:} $\Theta = \{\theta_t\}_{t=1}^T$ \\ $\left( \Rightarrow \hat{Q}_{t}^{\pi_t}(s,a) = f_{\theta_t}(s,a) \approx Q_{t}^{\pi_t}(s,a), \forall s,a \in \mathcal{S}\times \mathcal{A} \right) $
\end{algorithmic}
\end{algorithm}
% ===========================================================================================

